Characterizing Bugs in Python and R Data Analytics Programs

R and Python are among the most popular languages used in many critical data analytics tasks. However, we still do not fully understand the capabilities of these two languages w.r.t. bugs encountered in data analytics tasks. What type of bugs are common? What are the main root causes? What is the relation between bugs and root causes? How to mitigate these bugs? We present a comprehensive study of 5,068 Stack Overflow posts, 1,800 bug fix commits from GitHub repositories, and several GitHub issues of the most used libraries to understand bugs in R and Python. Our key findings include: while both R and Python have bugs due to inexperience with data analysis, Python see significantly larger data preprocessing bugs compared to R. Developers experience significantly more data flow bugs in R because intermediate results are often implicit. We also found changes and bugs in packages and libraries cause more bugs in R compared to Python while package or library misselection and conflicts cause more bugs in Python than R. While R has a slightly higher readability barrier for data analysts, the statistical power of R leads to a less number of bad performance bugs. In terms of data visualization, R packages have significantly more bugs than Python libraries. We also identified a strong correlation between comparable packages in R and Python despite their linguistic and methodological differences. Lastly, we contribute a large dataset of manually verified R and Python bugs.

==> ChartsRPython.tex <==
\begin{figure}[h]
	\includegraphics[width=4.2in,trim={1.7cm 4.9cm 1cm 2cm},clip]{Charts-RvsPython.pdf}
	\caption{Type of different bugs with respect to root causes in R and Python}   
	\label{fig:RvsPython}
\end{figure}

==> LB_r.tex <==
As an example of logic bug is shown below.
A question\footnote{\url{https://bit.ly/31vfJv4}} asked in \sof about the 
wrong result of the \dplyr query written in R:

\begin{lstlisting}[language = r]
value <- mydata$value
qu25 <- mydata %>% 
	group_by(month, day, station_number) %>% 
	arrange(desc(value)) %>% 
	slice(3) %>% 
	select(value)
\end{lstlisting}

An answer by an expert that was accepted by an R developer who posted this question suggested:

\begin{lstlisting}[language = r]
qu25 <- mydata %>% 
	group_by(month, day, station_number) %>%
	arrange(desc(value)) %>% 
	slice(2) %>% 
	ungroup() %>%
	select(value)
\end{lstlisting}

==> LBnewExample.tex <==
For example, replacing the missing values, i.e. NaN, can lead to a bug in Python when using \textit{.isnan} from Math module and the \pandas \textit{.replace} as mentioned in the \sof post~\cite{13295735}. 
%The data frame could be fixed as follows:  
%\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python]
%df[1].fillna(0, inplace=True)
%\end{lstlisting}
Similarly in R a developer tried to replace NaN values with zeros; however, got confused with \textit{is.nan} as follows that led to a bug~\cite{18142117}:
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = R, numbers=left]
rapply(data123, f=function(x) ifelse(is.nan(x),0,x), how="replace")
\end{lstlisting}
To fix this bug, developer could use \textit{is.nan} as follows:   
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = R, numbers=left]
is.nan.data.frame <- function(x)
do.call(cbind, lapply(x, is.nan))
data123[is.nan(data123)] <- 0
\end{lstlisting}
Python developers have support for the extraction, transformation, and loading data automatically through ETL packages e.g., \textit{petl}~\cite{petl}, \textit{pygramet}~\cite{pygrametl}. 
For instance, loading CSV file and replace empty values with 0 can simply be done together using only this line~\cite{43723225}:
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python, numbers=left]
tb_probii = etl.fromcsv("data.csv").replace("score", "", 0)
\end{lstlisting}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> acknowledgements.tex <==
\section{Acknowledgements}
This project was supported in part by XXXXX.XXXXX.XXXXX.
We thank SeokHwan Song and Yijia Huang for data collection efforts.
Any opinions, findings, and conclusions or recommendations
expressed in this material are those of the authors and do not
necessarily reflect the views of the sponsors.



==> bugfig.tex <==
\begin{figure}[h]
    \includegraphics[width=3.6in,trim={0cm 4.8cm 0cm 4cm},clip]{figures/combinedbug.pdf}
    %    \includegraphics[keepaspectratio = True, scale = .4, trim={0cm 5cm 0cm 6cm},clip]{figures/BugTypes_Python.pdf}
    \caption{Bug types of Python and R in \sof}   
    \label{fig:typesRPython}
\end{figure}


%\begin{figure}[h]
%	\includegraphics[width=3.2in,trim={0.5cm 0.5cm 0cm 0.5cm},clip]{figures/BugTypes-Python.pdf}
%	%    \includegraphics[keepaspectratio = True, scale = .4, trim={0cm 5cm 0cm 6cm},clip]{figures/BugTypes_Python.pdf}
%	\caption{Bug types of Python in \sof dataset}   
%	\label{fig:1}
%\end{figure}
%
%
%\begin{figure}[h]
%	\includegraphics[width=3.2in,trim={0.5cm 0.5cm 0cm 0.5cm},clip]{figures/BugTypes-R.pdf}
%	\caption{Bug types of R in \sof dataset}   
%	\label{fig:2}
%\end{figure}

==> bugtypesRPython.tex <==
%\begin{figure*}[h!t]
%	\centering
%	\begin{subfigure}[t]{0.3\textwidth}
%		\centering
%		\includegraphics[height=1.1in]{Bug Types (R).pdf}
%		\caption{Bug Types (R)}
%	\end{subfigure}\qquad	
%	\begin{subfigure}[t]{0.3\textwidth}
%		\centering
%		\includegraphics[height=1.1in]{Bug Types (Python).pdf}
%		\caption{Bug Types (Python)}
%	\end{subfigure}\qquad	
%	\caption{Bug Types of R and Python}
%	\label{fig:tria}
%\end{figure*}
%






==> categoriesVSbugs.tex <==

\begin{figure}[h]
	\includegraphics[width=3.2in,trim={1cm 0.9cm 0cm 1.5cm},clip]{categoriesVSbugs.pdf}
	\caption{Bug types (\%) of Python and R in terms of categories}   
	\label{fig:categories}
\end{figure}

==> causeRPython.tex <==
\begin{figure}[h]
	\includegraphics[width=3.6in,trim={0cm 4.2cm 0cm 4cm},clip]{figures/combinedcause.pdf}
	%    \includegraphics[keepaspectratio = True, scale = .4, trim={0cm 5cm 0cm 6cm},clip]{figures/BugTypes_Python.pdf}
	\caption{Causes of Python and R bugs in \sof}   
	\label{fig:rootcausesPythonR}
\end{figure}







%\begin{figure}[h]
%	\includegraphics[width=3.2in,trim={0.5cm 0.5cm 0cm 0.5cm},clip]{figures/RootCause-Python.pdf}
%	\caption{Causes of Python bugs in \sof dataset}   
%	\label{fig:rootcausesPython}
%\end{figure}
%\begin{figure}[h]
%	\includegraphics[width=3.2in,trim={0.5cm 0.5cm 0cm 0.5cm},clip]{figures/RootCause-R.pdf}
%	\caption{Causes of R bugs in \sof dataset}   
%	\label{fig:rootcausesR}
%\end{figure}



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph*{\textbf{Implications for Practice} }  
Data science is the world's fastest-growing profession. However, it is challenging and there are lots of barriers for new talents to enter. This study introduces new data scientists to bugs, root causes behind bugs, and the bug effects of most used packages in R and Python that may help them in choosing the proper packages for their goals.


\paragraph*{\textbf{Software Engineering Research Implications} } 

While investigating the \sof and \gh dataset to address \textbf{RQ1}, we have realized that R's functional programming paradigm and Python's object-oriented paradigm that have caused different bugs in data analysis software. While loading data to memory and preparing it for the data science pipeline in R is easier due to the in-built features of R, the functional-based nature of the code makes it difficult for the developer to follow the data transformation steps. Intermediate results are stored implicitly which makes more data flow bugs that are difficult to fix.

While R has slightly readability challenge for data scientists to enter, the statistical power of R makes writing programs more efficient. We have seen that syntax error in \sof dataset for R developer is slightly higher than Python developers.


The taxonomy for root causes we proposed in this study, helps future researchers to identify the scale of changes and automatic tools to detect and remove some of the bugs generated by each cause. 


Both R and Python communities need a better verification tool and technique that makes the debugging code easier.

R and Python are the 2 different open source languages that are being used together. While data scientists mostly use R at the early stages of the data science pipeline, data engineers use Python at the later stages of the pipeline. This study would help both groups and provide a better understanding of the similar bugs they are making in building a data science pipeline and adapt a language-agnostic verification tool as well as technique to fix bugs efficiently.


\paragraph*{\textbf{Implications for Education} } There have been many discussions for learning data science for educators and which language to choose. This study from an education point of view facilitates this decision for different data analytics programs. Educators can utilize the results of our study to design the best curriculum as many universities and colleges are opening new data science majors. 


==> effectRPython.tex <==
\begin{figure}[h]
	\includegraphics[width=3.6in,trim={0cm 4.2cm 0cm 4cm},clip]{figures/combinedeffect.pdf}
	%    \includegraphics[keepaspectratio = True, scale = .4, trim={0cm 5cm 0cm 6cm},clip]{figures/BugTypes_Python.pdf}
	\caption{Effects of bugs for Python and R in \sof}   
	\label{fig:effectPythonR}
\end{figure}

%\begin{figure}[h]
%	\includegraphics[width=3.2in,trim={0.5cm 0.5cm 0cm 0.5cm},clip]{figures/Effect-Python.pdf}
%	\caption{Effects of bugs for Python in \sof dataset}   
%	\label{fig:effectsPython}
%\end{figure}
%\begin{figure}[h]
%	\includegraphics[width=3.2in,trim={0.5cm 0.5cm 0cm 0.5cm},clip]{figures/Effect-R.pdf}
%	\caption{Effects of bugs for R in \sof dataset}   
%	\label{fig:effectsR}
%\end{figure}

==> evolutionhistory.tex <==
%\begin{figure}[h]
%	\centering
%	\subfloat[]{{\includegraphics[scale= .36, trim={0cm 0cm 0cm 0cm},clip]{figures/numpyEvo.pdf} }}% 
%	\qquad
%	\subfloat[]{{\includegraphics[scale= .36,trim={0cm 0cm 0cm 0cm},clip]{figures/vizEvo.pdf} }}%
%	\caption{Evolution history of numpy, visualization packages of Python (matplotlib), and R (ggplot2) in response to the resolved Git Issues about API change and package/libraries update and version issues}%
%	\label{fig:evolution}%
%\end{figure}

\begin{figure}[h]
	\includegraphics[width=2.6in,trim={0cm 0cm 0.5cm 0.5cm},clip]{EvolutionFig.pdf}
%	\caption{Evolution history of numpy, visualization packages of Python (matplotlib), and R (ggplot2) in response to the resolved Git Issues about API change and package/libraries update and version issues}
	\caption{Evolution history of numpy, visualization package of Python (matplotlib), R (ggplot2) in response to resolved Git issues on API change, package update and version issues}   
	\label{fig:evolution}
\end{figure}

==> examples/CDApy.tex <==



==> examples/DAIpy.tex <==
%For instance, an efficient way is required to update the levels of a pandas MultiIndex after slicing its DataFrame posted by a developer~\cite{so28772494}. That issue can be resolved efficiently using the following code:

% \begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python, numbers=left]
% df.index.get_level_values(<levelname>)
% \end{lstlisting}
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = diff, numbers=left]
frame = pd.DataFrame(data)
- frame['HighScore'] = max(data['test1'], data['test2'], data['test3'])
+ frame['HighScore'] = frame[['test1','test2','test3']].max(axis=1)
\end{lstlisting}
To illustrate DAI, let us consider an example~\cite{20033111} as illustrated above, 
In this example, user wants to add a new column that shows the max value for each row. The user tries to pass each row to max() but it only works sometimes, and if there is another other way of doing it. According to an expert, the diff indicated on line 3 shows the efficient way to solve the problem. In another example as shown in a \sof post~\cite{24617356}, a developer needs to shuffle the training data between each iteration to efficiently use SGD to classify a large dataset.


==> examples/DAIr.tex <==
Similarly, R developer wants an efficient way to read different \textit{txt} files using \textit{fread}, and then union them into a bigger dataset posted by a developer~\cite{so21156271}. 
%The issue can be solved as follows: 
%in the following way.
%\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = r]	
%l <- lapply(all.files, fread, sep=",")
%dt <- rbindlist( l )
%setkey( dt , ID, date)
%\end{lstlisting}	

==> examples/DBPyR.tex <==
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python]
data = pd.DataFrame({"string_with_crlf": ["a\r\nbc"]})
with open("test2.csv", mode='w') as f:
data.to_csv(f, index=False)
\end{lstlisting}
We have observed the above Git issue of \textit{pandas-dev} ~\cite{gitissueCSV} in which developer gets unexpected output while using \textit{df.to\_csv()} for writing to an existing file handle without explicitly setting \textit{newline}. 
%='' (or newline='\textbackslash n') 
In the open statement an extra \lq \textbackslash r\rq is added to the default \lq\textbackslash r\textbackslash n\rq line-end on Windows.
%We have found this sort of issue in \sof~\cite{so3191528} as well.
However, the \textit{write.csv} function from the \textit{utils} package in R does not have such kind of issue.

%The solution would be to install 'xlrd' as mentioned by an expert with high reputation on \sof. 

%\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python]
%data = pd.DataFrame({"string_with_lf": ["a\nbc"], "string_with_crlf": ["a\r\nbc"]})
%with open("test2.csv", mode='w') as f:
%data.to_csv(f, index=False)
%with open("test2.csv", mode='rb') as f:
%print(f.read())
%\end{lstlisting}

==> examples/DFBPython.tex <==
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python]
items_counts = df['item'].value_counts()
max_item = items_counts.max()
\end{lstlisting}


==> examples/LBpy.tex <==
Similar scenario happens in Python, for example, in a similar task for data 
manipulation by \pandas, a developer posted a buggy code~\cite{so22751498}:

%TODO: this example for python for LB: https://stackoverflow.com/questions/41286569/get-total-of-pandas-column


\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python, numbers=left]
df.groupby('group')['a'].apply(sum(x > 0 for x in df['a']))
\end{lstlisting}

This code gets $AttributeError$. An answer posted by an expert suggested to modify steps of data manipulation 
that changes the logic of the program: 

%\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python]
%AttributeError: 'numpy.int32' object has no attribute 'module'
%\end{lstlisting}



\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python, numbers=left]
.agg({'pos':lambda ts: (ts > 0).sum()})
\end{lstlisting}

==> examples/LBr.tex <==
An example of such bug from \sof appears below 
where the query is about \dplyr.
% A question~\cite{so38511743} asked in \sof about the 
% wrong result of the \dplyr query:
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = r, numbers=left]
value <- mydata$value
qu25 <- mydata %>% 
	group_by(month, day, station_number) %>% 
	arrange(desc(value)) %>% 
	slice(3) %>% 
	select(value)
\end{lstlisting}
\change{An expert with high reputation in \sof provided following fixes that was accepted by a developer who posted this question:}
\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = r, numbers=left]
qu25 <- mydata %>% 
	group_by(month, day, station_number) %>%
	arrange(desc(value)) %>% 
	slice(2) %>% 
	ungroup() %>%
	select(value)
\end{lstlisting}

==> rq5.tex <==
\section{RQ5: Evolution of data analytics packages}
\label{sec:rq5}
%\finding{Package/libraries update related and version issues are prevalent more 
%than API change issues over last few years.}
\input{evolutionhistory.tex}
We also investigated the evolution history of Python and R libraries by obtaining the
number of releases were made and inspecting how libraries' versions have been 
released in response to the resolved Git Issues over last eight years. 
We found package/libraries update related and version issues are prevalent more 
than API change issues in this period. 
The evolution history of most released library of Python, numpy (101 releases~\cite{numpyEvo}), 
as well as visualization packages of Python (matplotlib with 86 releases~\cite{matplotlibEvo}), 
and R (ggplot2 with 36 releases~\cite{ggplot2Evo}) in response to the resolved Git Issues 
regarding API change (APIC) and Package/Library Mis-selection and Conflicts(PLMC) 
has been depicted in \figref{fig:evolution}. 
Developers, in some cases, are not aware of these dependencies and issues that are caused by new versions. 

\textbf{Implication: }
\textit{Library developers should be aware of the change rate of such packages to inform the practitioners about the root causes to reduce issues with those packages. There is a need for studies to identify root causes and build tools to automatically detect issues with API version changes during the execution of data analytics code.}









==> rq6.tex <==
\section{Which Tasks in \DS Programs are the Most Afflicted by Bugs?}
\label{sec:rq6}

To address \textbf{RQ6}, we categorized top used packages in R and Python according to similar functionality into four categories: data acquisition, data manipulation, mathematical functions, machine learning, and data visualization. Some libraries cover several functionalities. To remedy this, in the manual process, we removed irrelevant posts. For example, we did not consider posts for DNN training in the visualization category. We did not have enough data points to compare like-to-like packages.

%Comparison of bug types with respect to root causes for different stages 
%of DS pipeline in R and Python has been demonstrated in \figref{fig:RvsPython}.

\input{categoriesVSbugs}


%\subsection{Data Acquisition}

%\subsection{Data Manipulation}

\subsection{Data Manipulation and Mathematical Function and Machine Learning}
\change{
\finding{Python packages for data manipulation and Mathematical Function \& Machine Learning steps are more affected by bugs than that similar R packages.}

For data manipulation, Python packages show approximately 35\% of bugs. Similar R packages have approximately 25\% of such bugs. For mathematical functions and machine learning (ML), Python shows {\bf 24.80}\% of bugs while for similar tasks R has {\bf5.79}\% of bugs as shown in \figref{fig:categories}. These findings demonstrate the popularity of Python to solve those ML tasks; Bug detection tools can focus on these use cases and the unique challenges of finding and fixing ML bugs. Also, Python educators can focus on those steps when guiding new developers.
}
%%This is not a surprise due to the statistical power of R that is built for statisticians. 
%%implications Would it's be best fit for FInding 7?
%From our observation in terms of using mathematical and machine learning package, other than CDA and DAI that discussed in the previously, IDAP is another major root cause of bugs in DS programs. 
%An automated tool that utilizes the API documentation would ensure that APIs meet the constraints defined in the specifications. In this context, 
%Huang~\etal proposed an automatic approach ~\cite{huang2018api} to recommend APIs based on API documentation and StackOverflow posts.
%
%%Python provides mathematical packages for the developers to solve a mathematical problem easily. The developers need to go through all the list of packages to know about the useful functions for a particular problem. Sometimes, the developers made mistakes, e.g., incorrect number and order of parameters, and missing package import while using the APIs, which cause bugs in the program. To avoid these kinds of bugs, an automated tool could have been very much helpful. An automated API tool can solve this kind of problem and ensure that APIs meet the constraints defined in the specifications. Although there exists work related to API method recommendation \cite{}, a pragmatic tool that can recommend API correctly in DS programs written using R and Python.

\subsection{Data Visualization}

\finding{R packages for the data visualization step have the most bugs, when compares to other steps.}
\change{
Data visualization packages in R have {\bf 46.99}\% of bugs while 
similar packages in Python have {\bf 23.80}\% of bugs in Python.
We further investigated this issue by analyzing the visualization approach taken by both languages. The \ggplot package utilizes a layered approach to generate plots by which developers can add different aesthetics and layers. The layered approach tends to have more initialization and data flow bugs by writing more codes, while \matplotlib provides classes that developers can use to generate different plots. Incorrect functionality of plots in \ggplot causes the most bugs effects in R programs, making it very difficult for developers to localize bugs.
For example, an R developer tried to make a chart, and got an unexpected chart~\cite{so10660775}:}
  \begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = r]    
a + geom_bar() + 
  geom_bar(colour="black",show_guide=FALSE) +
  scale_fill_manual(values=c("white", "black"))
\end{lstlisting} 
An expert suggested adding another layer to fix the chart.
 \begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = r]  
  opts(legend.key = theme_rect(fill = 'black'))
\end{lstlisting} 
%TODO: can we refer to tableau? Or is there a declarative technique for visualization?
\change{These findings motivate the need for new tools and techniques for finding and fixing bugs in data visualization software. By ensuring the correctness of data visualization tools, developers can arrive solutions best fitted to their problem. Also, being able to detect data inconsistencies early in the { \color{red}Data Science} pipeline~\textbf{CITE}.
}


% By enabling the correctness of the data visualization tool, developers can arrive better solutions to their 

% the popularity of Python to solve those ML tasks; Bug detection tools can focus on these use cases and the unique challenges of finding and fixing ML bugs. Also, Python educators can focus on those steps when guiding new developers.

%This finding suggests that a better visualization support is needed.
%One approach would be declarative techniques, such as ~\cite{ni2017substance} for mathematical diagrams.
%Another potential approach would be to use an automatic tool and would help data scientists to spend less time on localizing and repairing bugs. 
%AutoViz~\cite{autoViz} is a data visualization Python library which automatically visualizes dataset with code which can reduce possibility of bugs in data visualization program written in Python. Such kind of tool for R can be useful to mitigate bugs caused in visualizing data analysis output.

%TODO: check if there is such a recent tool for R?

==> tables/bugtype.tex <==
%\begin{table*}
%	\vspace{15pt}
%	\centering
%	\caption{Statistics of Bug Types in \sof and \gh}
%	\label{tbl:gitsobugs}
%	\setlength{\tabcolsep}{0.5pt}
%	\footnotesize
%	\renewcommand{\arraystretch}{0.5}
%	\begin{tabular}{|p{3cm}|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		\multirow{2}{*}{}             		& \multicolumn{2}{c|}{ggplot2} & \multicolumn{2}{c|}{dplyr} 	& \multicolumn{2}{c|}{shiny} 	& \multicolumn{2}{c|}{data.table}	& \multicolumn{2}{c|}{rmarkdown} &	\multicolumn{2}{c|}{matrix} 		 		 	& \multirow{2}{*}{P value}\\ \cline{2-11} 
%		& \rotatebox[origin=c]{90} {SO}  & \rotatebox[origin=c]{90} {GitHub}  & \rotatebox[origin=c]{90} {SO}   & \rotatebox[origin=c]{90} {GitHub}        & \rotatebox[origin=c]{90} {SO}       &\rotatebox[origin=c]{90} {GitHub}        & \rotatebox[origin=c]{90} {SO}       &
%		\rotatebox[origin=c]{90} {GitHub}       & \rotatebox[origin=c]{9z0} {SO} & \rotatebox[origin=c]{90} {SO}       &\rotatebox[origin=c]{90} {GitHub}      &
%		\rotatebox[origin=c]{90} {GitHub}       & \\ \hline

%		API Bug                       		 &   & 		&  & 	&  &  &  & &  &  &  & &  \\ \hline

%	\end{tabular}
%\vspace{-15pt}
%\end{table*}

% Table generated by Excel2LaTeX from sheet 'BugtypeTable'
\begin{table*}[htbp]
	%\footnotesize
	%\scriptsize
	\fontsize{6.6}{6.6}\selectfont
	\centering
	\caption{Bug types}
	\setlength{\tabcolsep}{0.6pt}
	\begin{tabular}{|p{4.82em}|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{4}[8]{*}{\textbf{Bug Types}} & \multicolumn{4}{c|}{\textbf{Data Acquisition}} & \multicolumn{6}{c|}{\textbf{Data Manipulation}} & \multicolumn{14}{c|}{\textbf{Mathematical function and Machine Learning}}      & \multicolumn{12}{c|}{\textbf{Data Visualization}} \\
		\hline    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{\textbf{R}} & \multicolumn{2}{c|}{
			\textbf{Python}} & \multicolumn{4}{c|}{
			\textbf{R}} & \multicolumn{2}{c|}{
			\textbf{Python}} & \multicolumn{8}{c|}{
			\textbf{R}} & \multicolumn{6}{c|}{
			\textbf{Python}} & \multicolumn{8}{c|}{
			\textbf{R}} & \multicolumn{4}{c|}{
			\textbf{Python}} \\
		\hline    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{data.table}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{dataframe}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{dplyr}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{tidyr}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{pandas}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{matrix}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{randomforest}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{r-caret}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{time-series}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{numpy}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{scipy}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{scikit-learn}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{ggplot2}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{plotly}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{shiny}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{igraph}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{matplotlib}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{pyqt}}} \\
		\hline    \multicolumn{1}{|r|}{} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} \\
		
		\hline
		\textbf{IIS} & 21\%  & 14\%  & 4\%   & 10\%  & 19\%  & 11\%  & 22\%  & 0\%   & 8\%   & 5\%   & 0\%   & 15\%  & 7\%   & 5\%   & 18\%  & 7\%   & 0\%   & 0\%   & 14\%  & 6\%   & 35\%  & 6\%   & 19\%  & 11\%  & 15\%  & 16\%  & 17\%  & 5\%   & 24\%  & 12\%  & 0\%   & 16\%  & 22\%  & 7\%   & 32\%  & 9\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{CB} & 6\%   & 0\%   & 3\%   & 8\%   & 4\%   & 3\%   & 0\%   & 10\%  & 2\%   & 10\%  & 0\%   & 0\%   & 0\%   & 5\%   & 0\%   & 2\%   & 0\%   & 4\%   & 1\%   & 7\%   & 0\%   & 5\%   & 0\%   & 7\%   & 3\%   & 4\%   & 0\%   & 5\%   & 10\%  & 7\%   & 0\%   & 13\%  & 2\%   & 10\%  & 0\%   & 7\% \\
		%\hline
		\textbf{DB} & 2\%   & 0\%   & 31\%  & 5\%   & 1\%   & 0\%   & 0\%   & 0\%   & 14\%  & 3\%   & 12\%  & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 2\%   & 12\%  & 2\%   & 7\%   & 4\%   & 9\%   & 1\%   & 1\%   & 0\%   & 0\%   & 0\%   & 0\%   & 2\%   & 0\%   & 0\%   & 3\%   & 1\%   & 2\%   & 2\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{CFB} & \cellcolor[rgb]{ .8,  .8,  .8}1\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}2\% & \cellcolor[rgb]{ .8,  .8,  .8}13\% & \cellcolor[rgb]{ .8,  .8,  .8}2\% & \cellcolor[rgb]{ .8,  .8,  .8}9\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}10\% & \cellcolor[rgb]{ .8,  .8,  .8}1\% & \cellcolor[rgb]{ .8,  .8,  .8}17\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}12\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}5\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}12\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}2\% & \cellcolor[rgb]{ .8,  .8,  .8}2\% & \cellcolor[rgb]{ .8,  .8,  .8}11\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}10\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}11\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}10\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}5\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}14\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}3\% & \cellcolor[rgb]{ .8,  .8,  .8}2\% & \cellcolor[rgb]{ .8,  .8,  .8}15\% & \cellcolor[rgb]{ .8,  .8,  .8}0\% & \cellcolor[rgb]{ .8,  .8,  .8}14\% \\
		%\hline
		\textbf{DFB} & 10\%  & 0\%   & 7\%   & 3\%   & 27\%  & 0\%   & 22\%  & 0\%   & 17\%  & 2\%   & 8\%   & 3\%   & 47\%  & 2\%   & 27\%  & 0\%   & 6\%   & 5\%   & 16\%  & 0\%   & 3\%   & 3\%   & 9\%   & 1\%   & 15\%  & 0\%   & 0\%   & 2\%   & 2\%   & 5\%   & 17\%  & 0\%   & 1\%   & 2\%   & 0\%   & 2\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{IB} & 9\%   & 62\%  & 3\%   & 16\%  & 2\%   & 11\%  & 0\%   & 60\%  & 6\%   & 17\%  & 8\%   & 29\%  & 13\%  & 33\%  & 9\%   & 41\%  & 13\%  & 40\%  & 4\%   & 25\%  & 2\%   & 25\%  & 0\%   & 17\%  & 16\%  & 26\%  & 25\%  & 33\%  & 15\%  & 19\%  & 17\%  & 19\%  & 4\%   & 19\%  & 0\%   & 21\% \\
		%\hline
		\textbf{LB} & 44\%  & 24\%  & 43\%  & 35\%  & 41\%  & 57\%  & 56\%  & 20\%  & 48\%  & 40\%  & 73\%  & 35\%  & 33\%  & 47\%  & 45\%  & 36\%  & 81\%  & 47\%  & 47\%  & 45\%  & 52\%  & 36\%  & 58\%  & 45\%  & 45\%  & 42\%  & 50\%  & 47\%  & 46\%  & 33\%  & 67\%  & 47\%  & 62\%  & 39\%  & 60\%  & 37\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{PB} & 6\%   & 0\%   & 8\%   & 10\%  & 4\%   & 9\%   & 0\%   & 0\%   & 4\%   & 6\%   & 0\%   & 5\%   & 0\%   & 4\%   & 0\%   & 2\%   & 0\%   & 0\%   & 4\%   & 4\%   & 2\%   & 11\%  & 5\%   & 7\%   & 5\%   & 2\%   & 8\%   & 4\%   & 2\%   & 7\%   & 0\%   & 3\%   & 4\%   & 7\%   & 6\%   & 8\% \\
		\hline	
	\end{tabular}%
	\label{tab:bugtypes}%
	\footnotesize * %\textbf{\textcolor{green}{Green}}
	Interface, Integration, and System Bugs (IIS), Coding Bugs (CB),Data Bugs (DB), 
	Control Flow Bugs (CFB), Data flow Bugs (DFB), \\ Initialization Bugs (IB), Logic Bugs (LB), Processing Bugs (PB), GitHub (GH), StackOverflow (SO)
\end{table*}%


==> tables/effects.tex <==
% Table generated by Excel2LaTeX from sheet 'BugtypeTable'
\begin{table*}[htbp]
	%\footnotesize
	%\tiny
	\fontsize{6.6}{6.6}\selectfont
	\centering
	\caption{Effects}
	\setlength{\tabcolsep}{0.8pt}
	\begin{tabular}{|p{4.82em}|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{4}[8]{*}{\textbf{Effects}} & \multicolumn{4}{c|}{  \textbf{Data Acquisition}} & \multicolumn{6}{c|}{  \textbf{Data Manipulation}} & \multicolumn{14}{c|}{ \textbf{Mathematical function and Machine Learning}}      & \multicolumn{12}{c|}{  \textbf{Data Visualization}} \\
		\hline    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{  \textbf{R}} & \multicolumn{2}{c|}{  \textbf{Python}} & \multicolumn{4}{c|}{  \textbf{R}} & \multicolumn{2}{c|}{  \textbf{Python}} & \multicolumn{8}{c|}{\textbf{R}} & \multicolumn{6}{c|}{ \textbf{Python}} & \multicolumn{8}{c|}{  \textbf{R}} & \multicolumn{4}{c|}{  \textbf{Python}} \\
		\hline    \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{data.table}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{dataframe}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{dplyr}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{tidyr}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{pandas}}} & \multicolumn{2}{c|}{\rotatebox[origin=c]{90}{\textbf{matrix}}} & \multicolumn{2}{c|}{\rotatebox[origin=c]{90}{\textbf{randomforest}}} & \multicolumn{2}{c|}{\rotatebox[origin=c]{90}{\textbf{r-caret}} }& \multicolumn{2}{c|}{\rotatebox[origin=c]{90}{\textbf{time-series}}} & \multicolumn{2}{c|}{ \rotatebox[origin=c]{90}{\textbf{numpy}}} & \multicolumn{2}{c|}{ \rotatebox[origin=c]{90}{\textbf{scipy}}} & \multicolumn{2}{c|}{ \rotatebox[origin=c]{90}{\textbf{scikit-learn}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{ggplot2}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{plotly}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{shiny}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{igraph}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{matplotlib}}} & \multicolumn{2}{c|}{  \rotatebox[origin=c]{90}{\textbf{pyqt}}} \\
		\hline    \multicolumn{1}{|r|}{} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &  \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &  \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{SO}}} &   \rotatebox[origin=c]{90}{\textit{\textbf{GH}}} \\
		\hline
		
		\textbf{BP} & 10\%  & 0\%   & 7\%   & 4\%   & 3\%   & 0\%   & 11\%  & 0\%   & 10\%  & 2\%   & 23\%  & 5\%   & 27\%  & 0\%   & 9\%   & 0\%   & 13\%  & 0\%   & 16\%  & 2\%   & 7\%   & 3\%   & 3\%   & 0\%   & 0\%   & 0\%   & 8\%   & 0\%   & 2\%   & 0\%   & 0\%   & 3\%   & 4\%   & 0\%   & 2\%   & 3\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{Crash} & 59\%  & 52\%  & 58\%  & 63\%  & 75\%  & 71\%  & 22\%  & 50\%  & 58\%  & 44\%  & 27\%  & 75\%  & 60\%  & 57\%  & 73\%  & 66\%  & 31\%  & 67\%  & 58\%  & 43\%  & 57\%  & 35\%  & 73\%  & 52\%  & 56\%  & 46\%  & 33\%  & 57\%  & 44\%  & 71\%  & 17\%  & 97\%  & 32\%  & 43\%  & 53\%  & 41\% \\
		%\hline
		\textbf{DC} & 14\%  & 0\%   & 1\%   & 0\%   & 15\%  & 14\%  & 44\%  & 0\%   & 5\%   & 0\%   & 15\%  & 2\%   & 7\%   & 14\%  & 0\%   & 7\%   & 38\%  & 2\%   & 5\%   & 0\%   & 2\%   & 0\%   & 1\%   & 0\%   & 1\%   & 4\%   & 0\%   & 14\%  & 5\%   & 10\%  & 17\%  & 0\%   & 0\%   & 0\%   & 2\%   & 0\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{Hang} & 2\%   & 0\%   & 1\%   & 1\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 4\%   & 0\%   & 0\%   & 4\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 4\%   & 0\%   & 0\%   & 0\%   & 0\%   & 1\%   & 0\%   & 2\%   & 0\% \\
		%\hline
		\textbf{IF} & 10\%  & 31\%  & 34\%  & 23\%  & 7\%   & 11\%  & 22\%  & 30\%  & 25\%  & 36\%  & 12\%  & 12\%  & 7\%   & 7\%   & 18\%  & 19\%  & 19\%  & 30\%  & 18\%  & 40\%  & 35\%  & 34\%  & 18\%  & 30\%  & 43\%  & 32\%  & 58\%  & 7\%   & 49\%  & 10\%  & 50\%  & 0\%   & 61\%  & 43\%  & 42\%  & 44\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{Unknown} & 0\%   & 17\%  & 0\%   & 10\%  & 0\%   & 3\%   & 0\%   & 20\%  & 0\%   & 19\%  & 0\%   & 6\%   & 0\%   & 18\%  & 0\%   & 9\%   & 0\%   & 2\%   & 0\%   & 15\%  & 0\%   & 28\%  & 0\%   & 18\%  & 0\%   & 18\%  & 0\%   & 18\%  & 0\%   & 10\%  & 0\%   & 0\%   & 0\%   & 15\%  & 0\%   & 13\% \\
		%\hline
		\textbf{MOB} & 4\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 2\%   & 0\%   & 19\%  & 1\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 4\%   & 0\%   & 0\%   & 0\%   & 4\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 17\%  & 0\%   & 2\%   & 0\%   & 0\%   & 0\% \\
		\hline
 
    \end{tabular}%
  \label{tab:effects}%
  \footnotesize \\
  Incorrect Functionality (IF), Bad Performance (BP), Data Corruption (DC), Memory Out of Bound (MOB), GitHub (GH), StackOverflow (SO)
  
  
\end{table*}%


==> tables/kappa.tex <==
\begin{table}[ht]
	\caption{Interpretation of Cohen's Kappa Coefficient}
	\small
	%\textwidth
	\label{tbl:kappa}
	\centering
	\begin{tabular}{|l|l|}
		\hline
		\textbf{Range} & \textbf{Agreement level} \\
		\hline
		0.00-0.20 & Slight agreement\\
		\hline
		0.21-0.40 & Fair agreement \\
		\hline
		0.41-0.60 & Moderate agreement\\
		\hline
		0.61-0.80 & Substantial agreement \\
		\hline
		0.81-1.00 & Perfect agreement \\
	   \hline
	\end{tabular}
\end{table}

%
%\hline
%New York Stock Exchange data & NYS & Each stock has around 3k tuples. 
%\\ 
%\hline
%CO2 (ppm) mauna loa, 1965-1980 & CO2 & This small dataset has around 200 tuples.
%\\
%\hline
%Annual velocity of money, 1869 to 1970 & MNV & It has 103 tuples.
%\\
%\hline
%Highest mean monthly level, Lake Michigan, 1860 to 1955 & LMI & Total 97 tuples. 
%\\
%\hline
%High and low water levels of the Amazon at Iquitos, 1962 – 1995 & AMZ & Total 37 tuples. 
%\\
%\hline
%Annual GNP deflator, U.S., 1889 to 1970 & GNP & Total 83 tuples.
%\\
 

==> tables/rootcause.tex <==
% Table generated by Excel2LaTeX from sheet 'BugtypeTable'
\begin{table*}[htbp]
	%\footnotesize
	%\tiny
	\fontsize{6.6}{6.6}\selectfont
	\centering
	\caption{Root causes}
	\setlength{\tabcolsep}{0.6pt}
	\begin{tabular}{|p{6.82em}|c|c|c|c|c|c|c|c|c|c|c|c|c|c|r|r|c|c|c|c|c|c|c|c|c|r|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{4}[8]{*}{\textbf{Root Causes}} & \multicolumn{4}{c|}{
			\textbf{Data Acquisition}} & \multicolumn{6}{c|}{
			\textbf{Data Manipulation}} & \multicolumn{14}{c|}{
			\textbf{Mathematical function and Machine Learning}}      & \multicolumn{12}{c|}{
			\textbf{Data Visualization}} \\
		\hline   \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{
			\textbf{R}} & \multicolumn{2}{c|}{
			\textbf{Python}} & \multicolumn{4}{c|}{
			\textbf{R}} & \multicolumn{2}{c|}{
			\textbf{Python}} & \multicolumn{8}{c|}{
			\textbf{R}} & \multicolumn{6}{c|}{
			\textbf{Python}} & \multicolumn{8}{c|}{
			\textbf{R}} & \multicolumn{4}{c|}{
			\textbf{Python}} \\
		\hline   \multicolumn{1}{|r|}{} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{data.table}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{dataframe}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{dplyr}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{tidyr}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{pandas}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{matrix}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{randomforest}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{r-caret}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{time-series}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{numpy}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{scipy}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{scikit-learn}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{ggplot2}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{plotly}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{shiny}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{igraph}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{matplotlib}}} & \multicolumn{2}{c|}{
			\rotatebox[origin=c]{90}{\textbf{pyqt}}} \\
		\hline   \multicolumn{1}{|r|}{} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & \multicolumn{1}{c|}{
			\rotatebox[origin=c]{90}{\textit{\textbf{SO}}}} & \multicolumn{1}{c|}{
			\rotatebox[origin=c]{90}{\textit{\textbf{GH}}}}& 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & \multicolumn{1}{c|}{
			\rotatebox[origin=c]{90}{\textit{\textbf{GH}}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} &
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{SO}}} & 
		\rotatebox[origin=c]{90}{\textit{\textbf{GH}}} \\
		\hline
		\textbf{AAC} & 1\%   & 0\%   & 0\%   & 0\%   & 2\%   & 0\%   & 0\%   & 0\%   & 0.6\% & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & \multicolumn{1}{c|}{0\%} & \multicolumn{1}{c|}{0\%} & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & \multicolumn{1}{c|}{0\%} & 0\%   & 0\%   & 2\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 1\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{TM} & 6\%   & 0\%   & 11\%  & 1\%   & 12\%  & 0\%   & 0\%   & 0\%   & 15\%  & 0\%   & 4\%   & 0\%   & 7\%   & 1\%   & \multicolumn{1}{c|}{9\%} & \multicolumn{1}{c|}{0\%} & 0\%   & 4\%   & 15\%  & 1\%   & 2\%   & 2\%   & 4\%   & 0\%   & 11\%  & \multicolumn{1}{c|}{0\%} & 0\%   & 1\%   & 0\%   & 5\%   & 17\%  & 0\%   & 3\%   & 1\%   & 0\%   & 0\% \\
		%\hline
		\textbf{APIC} & 14\%  & 3\%   & 3\%   & 1\%   & 11\%  & 11\%  & 11\%  & 0\%   & 4\%   & 0\%   & 0\%   & 0\%   & 7\%   & 0\%   & \multicolumn{1}{c|}{9\%} & \multicolumn{1}{c|}{3\%} & 0\%   & 0\%   & 2\%   & 0\%   & 0\%   & 0\%   & 8\%   & 2\%   & 9\%   & \multicolumn{1}{c|}{2\%} & 17\%  & 0\%   & 5\%   & 0\%   & 0\%   & 3\%   & 3\%   & 0\%   & 11\%  & 1\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{MRP} & 2\%   & 0\%   & 3\%   & 0\%   & 4\%   & 0.00\% & 0\%   & 10\%  & 1\%   & 1\%   & 0\%   & 0\%   & 0\%   & 0\%   & \multicolumn{1}{c|}{0\%} & \multicolumn{1}{c|}{0\%} & 0\%   & 0\%   & 0\%   & 0\%   & 3\%   & 0\%   & 3\%   & 1\%   & 2\%   & \multicolumn{1}{c|}{0\%} & 0\%   & 0\%   & 2\%   & 0\%   & 0\%   & 3\%   & 0\%   & 0\%   & 0\%   & 0\% \\
		%\hline
		\textbf{CDA} & 40\%  & 21\%  & 58\%  & 61\%  & 41\%  & 57\%  & 67\%  & 30\%  & 48\%  & 64\%  & 46\%  & 48\%  & 7\%   & 55\%  & \multicolumn{1}{c|}{36\%} & \multicolumn{1}{c|}{47\%} & 56\%  & 53\%  & 36\%  & 67\%  & 45\%  & 61\%  & 56\%  & 65\%  & 47\%  & \multicolumn{1}{c|}{52\%} & 42\%  & 55\%  & 54\%  & 52\%  & 50\%  & 50\%  & 56\%  & 63\%  & 66\%  & 65\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{IDAP} & 8\%   & 62\%  & 13\%  & 20\%  & 1\%   & 14\%  & 0\%   & 50\%  & 13\%  & 18\%  & 8\%   & 32\%  & 13\%  & 34\%  & \multicolumn{1}{c|}{9\%} & \multicolumn{1}{c|}{45\%} & 13\%  & 39\%  & 7\%   & 17\%  & 3\%   & 24\%  & 9\%   & 14\%  & 14\%  & \multicolumn{1}{c|}{28\%} & 25\%  & 34\%  & 12\%  & 24\%  & 17\%  & 16\%  & 12\%  & 19\%  & 0\%   & 18\% \\
		%\hline
		\textbf{DAI} & 13\%  & 0\%   & 6\%   & 0\%   & 3\%   & 0\%   & 11\%  & 0\%   & 10\%  & 2\%   & 31\%  & 2\%   & 27\%  & 0\%   & \multicolumn{1}{c|}{9\%} & \multicolumn{1}{c|}{0\%} & 13\%  & 0\%   & 15\%  & 2\%   & 7\%   & 1\%   & 3\%   & 0\%   & 0\%   & \multicolumn{1}{c|}{0\%} & 8\%   & 0\%   & 2\%   & 0\%   & 0\%   & 3\%   & 4\%   & 0\%   & 2\%   & 1\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{SM} & 2\%   & 0\%   & 4\%   & 1\%   & 14\%  & 0\%   & 0\%   & 0\%   & 4\%   & 1\%   & 8\%   & 3\%   & 40\%  & 0\%   & \multicolumn{1}{c|}{18\%} & \multicolumn{1}{c|}{0\%} & 6\%   & 2\%   & 12\%  & 1\%   & 5\%   & 2\%   & 6\%   & 0\%   & 5\%   & \multicolumn{1}{c|}{0\%} & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\% \\
		%\hline
		\textbf{WD} & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & \multicolumn{1}{c|}{0\%} & \multicolumn{1}{c|}{0\%} & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 1\%   & 0\%   & 1\%   & \multicolumn{1}{c|}{0\%} & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 1\%   & 0\%   & 0\%   & 0\% \\
		%\hline
		\rowcolor[rgb]{ .851,  .851,  .851} \textbf{Others} & 10\%  & 0\%   & 3\%   & 8\%   & 5\%   & 6\%   & 0\%   & 10\%  & 4\%   & 9\%   & 0\%   & 8\%   & 0\%   & 5\%   & 9\%   & 2\%   & 0\%   & 4\%   & 8\%   & 6\%   & 5\%   & 5\%   & 2\%   & 7\%   & 7\%   & 8\%   & 0\%   & 5\%   & 15\%  & 10\%  & 0\%   & 13\%  & 5\%   & 10\%  & 9\%   & 7\% \\
		%\hline
		\textbf{PLMC} & 3\%   & 14\%  & 3\%   & 9\%   & 8\%   & 11\%  & 11\%  & 0\%   & 1\%   & 5\%   & 4\%   & 8\%   & 0\%   & 5\%   & 0\%   & 3\%   & 13\%  & 0\%   & 6\%   & 6\%   & 30\%  & 6\%   & 8\%   & 10\%  & 3\%   & 10\%  & 8\%   & 5\%   & 7\%   & 10\%  & 17\%  & 13\%  & 16\%  & 7\%   & 11\%  & 8\% \\
		\hline      
    \end{tabular}%
  \label{tab:rootcauses}%
  \footnotesize \\
  Absence of Inter API Compatibility (AAC), Package or Library misselection and Conflicts (PLMC), API Change (APIC), Wrong Documentation (WD), Shape Mismatch (SM), Type Mismatch (TM), Incorrect Data Analysis Parameters (IDAP), Misuse Required Parameter (MRP), Confusion with Data Analysis (CDA), Data Analysis Inefficiency (DAI)
\end{table*}%


==> ttest.tex <==

\begin{table}[h]
    \footnotesize
	\centering
	\caption{P-value of the distribution of Bugs btween the libraries}
	\rowcolors{2}{gray!25}{white}
	\begin{tabular}{|  l  |  r |  r |  r |  r | r |}
		\hline
	\rowcolor{gray!50}
    Library & \caffe & \keras & \tensor & \theano & \torch \\
    \hline
    \caffe & 1.0 & 0.0045 & 0.00735 & 0.19 & 0.30\\
    \hline
    \keras & 0.0045 & 1.0  & 0.84 & 0.0021 & 0.0024 \\
    \hline
    \tensor & 0.0073 & 0.84  & 1.0 & 0.0039 & 0.0044 \\
    \hline
    \theano & 0.19 & 0.0021  & 0.0039 & 1.0 & 0.80 \\
    \hline
    \torch & 0.30 & 0.0024  & 0.0044 & 0.80 & 1.0 \\
    \hline
\end{tabular}
	\label{tbl:ttest}
\end{table}


